Learning from, Understanding, and Supporting DevOps Artifacts for Docker

With the growing use of DevOps tools and frameworks, there is an increased need for tools and techniques that support more than code. The current state-of-the-art in static developer assistance for tools like Docker is limited to shallow syntactic validation. We identify three core challenges in the realm of learning from, understanding, and supporting developers writing DevOps artifacts: (i) nested languages in DevOps artifacts, (ii) rule mining, and (iii) the lack of semantic rule-based analysis. To address these challenges we introduce a toolset, binnacle, that enabled us to ingest 900,000 GitHub repositories. Focusing on Docker, we extracted approximately 178,000 unique Dockerfiles, and also identified a Gold Set of Dockerfiles written by Docker experts. We addressed challenge (i) by reducing the number of effectively uninterpretable nodes in our ASTs by over 80% via a technique we call phased parsing. To address challenge (ii), we introduced a novel rule-mining technique capable of recovering two-thirds of the rules in a benchmark we curated. Through this automated mining, we were able to recover 16 new rules that were not found during manual rule collection. To address challenge (iii), we manually collected a set of rules for Dockerfiles from commits to the files in the Gold Set. These rules encapsulate best practices, avoid docker build failures, and improve image size and build latency. We created an analyzer that used these rules, and found that, on average, Dockerfiles on GitHub violated the rules five times more frequently than the Dockerfiles in our Gold Set. We also found that industrial Dockerfiles fared no better than those sourced from GitHub. The learned rules and analyzer in binnacle can be used to aid developers in the IDE when creating Dockerfiles, and in a post-hoc fashion to identify issues in, and to improve, existing Dockerfiles.

==> overview.tex <==
\section{Overview}%
\label{Se:Overview}

The \texttt{binnacle} tool primarily operates in two distinct modes: in Mode I,
\texttt{binnacle} can be used to ingest arbitrary GitHub repositories and
extract a corpus of files from these repositories; in Mode II, \texttt{binnacle}
can be used to learn rules from a corpus of input files---following this, the
learned rules are fed to a static rule-enforcement engine to detect and catalog
violations. \Cref{Fi:Overview} depicts both of these modes of operation.

Mode I is the essential setup and data collection necessary to
drive the more interesting processing performed in Mode II. \Cref{Se:DataAcquisition}
describes Mode I (setup and collect) in greater detail.
The \texttt{binnacle} tool makes a distinction between Mode I and Mode II to allow
for other usages beyond the analysis we have done. Mode I is of broad use
to anyone looking to analyze vast swaths of GitHub data.

Mode II is the driver for rule learning and enforcement. Within Mode II there
are three key components: (i) phased parsing, (ii) rule mining,
and (iii) the rule-enforcement engine. Component (i), phased parsing, is a technique
we have developed to address the challenge of nested languages in DevOps artifacts.
This technique amounts to chaining various, increasingly specific, parsers together
to build an end-to-end parsing infrastructure capable of deriving rich ASTs from
input source files. This technique, although applied to Dockerfiles, is general in its
application to any DevOps artifacts with embedded shell. The only prerequisite is
the availability of a top-level parser. \Cref{Se:PhasedParsing} describes the
phased parsing technique in greater detail, and \Cref{Se:ResultsPhasedParsing}
presents a quantatative evaluation of \texttt{binnacle}'s phased parser.

Component (ii), rule mining, takes general tree-structured data as input and a
set of node types of interest. For each input node type, the rule miner finds
the set of sub-trees rooted at that node and applies a frequent sub-tree miner.
The outputs of the frequent sub-tree miner are then used to build simple rules.
\Cref{Se:TARs} presents further details on our rule encoding and \Cref{Se:RuleMining}
provides an in depth description of our rule mining technique. \Cref{Se:ResultsRules}
presents a comparative analysis of rule violations on the Gold Set and a set of
a random subset of Dockerfiles sampled from our Dockerfile corpus (see \Cref{Se:DataAcquisition}
for details on the methods used to collect our Dockerfiles corpus and identify
a Gold Set of high-quality Dockerfiles).

Lastly, component (iii), rule enforcement, takes a corpus of input trees
and a set of input rules, and reports all violations of the input rules. This
simple rule-based enforcement is only possible because of the phased parsing
performed earlier. Without rich representations, a simple rule-based analysis
would not yield sufficiently precise results. Furthermore, the simplicity
of the rule-enforcement engine allows for the rule miner to directly produce
rules (TARs), automatically, that can be fed into the rule-enforcement engine. \Cref{Se:Enforcement}
describes the details of our rule-enforcement engine, and the semantics of
the rules introduced in \Cref{Se:TARs} in greater detail.

% Local Variables:
% TeX-master: "paper.tex"
% End:
